Learned Monocular Depth Priors in Visual-Inertial Initialization

Visual-inertial odometry (VIO) is the pose estimation backbone for most AR/VR and autonomous robotic systems today, in both academia and industry. However, these systems are highly sensitive to the initialization of key parameters such as sensor biases, gravity direction, and metric scale. In practical scenarios where high-parallax or variable acceleration assumptions are rarely met (e.g. hovering aerial robot, smartphone AR user not gesticulating with phone), classical visual-inertial initialization formulations often become ill-conditioned and/or fail to meaningfully converge. In this paper we target visual-inertial initialization specifically for these low-excitation scenarios critical to in-the-wild usage. We propose to circumvent the limitations of classical visual-inertial structure-from-motion (SfM) initialization by incorporating a new learning-based measurement as a higher-level input. We leverage learned monocular depth images (mono-depth) to constrain the relative depth of features, and upgrade the mono-depths to metric scale by jointly optimizing for their scales and shifts. Our experiments show a significant improvement in problem conditioning compared to a classical formulation for visual-inertial initialization, and demonstrate significant accuracy and robustness improvements relative to the state-of-the-art on public benchmarks, particularly under low-excitation scenarios. We further extend this improvement to implementation within an existing odometry system to illustrate the impact of our improved initialization method on resulting tracking trajectories.

==> Figures/different_hz_study.tex <==
\begin{table}[!htbp]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}c c c c c c c@{}} \toprule
\multirow{2}{*}{\textbf{Metrics}}& \multicolumn{3}{c}{$10$KFs $10Hz$} & \multicolumn{3}{c}{$10$KFs $4Hz$} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
& \textbf{Intertial-Only} & \textbf{Baseline} & \textbf{Ours} & \textbf{Intertial-Only} & \textbf{Baseline} & \textbf{Ours} \\
\midrule
\midrule
\multicolumn{1}{l}{Scale Error (\%) ${\bar{|| a ||}} > 0.005G$}  & 35.67 & 16.36 & \textbf{13.78} & 14.65	& 8.76 & \textbf{8.41}\\
\cmidrule(lr){1-1}\cmidrule(lr){2-7}
\multicolumn{1}{l}{Position RMSE (meters)} & 0.123 & 0.038 & \textbf{0.034} & 0.066 & \textbf{0.061} & 0.064\\
\cmidrule(lr){1-1}\cmidrule(lr){2-7}
\multicolumn{1}{l}{Gravity RMSE (degrees)} & 1.89 & 1.42 & \textbf{1.38} & 1.36 & \textbf{1.32} & 1.36 \\
% \cmidrule(lr){1-1}\cmidrule(lr){2-7}
% \multicolumn{1}{l}{Mean Initialization Latency (seconds)} & 1.37 & \textbf{0.90} & \textbf{0.90} & \textbf{2.23} & 2.25 & 2.25 \\
\cmidrule(lr){1-1}\cmidrule(lr){2-7}
\multicolumn{1}{l}{\textbf{$\log$(Condition Num)} ${\bar{|| a ||}} < 0.005G$} & n/a & 12.12 & \textbf{11.23} & n/a &\textbf{10.25} & 10.54 \\

\bottomrule
\end{tabular}
}
\caption{Aggregated initialization benchmark for Inertial-Only, Baseline and our proposed method using various framerates on all EuRoC datasets. For each metric, lower is better.}
\label{different hz study}
\end{table}

==> Figures/mean_error_wrt_gt_dist.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{Figures/mean-error-wrt-gt-dist.png}
    \caption{Mean Initailization Errors w.r.t Ground Truth Camera Distance. Growing error w.r.t wider baseline in EuRoC is often due to large, constant velocities which have poor observ-ability}
    \label{fig:vio-evaluation}
\end{figure}


==> Figures/vio_eval_fig.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{Figures/VIO Evaluation.png}
    \caption{$10$ second VIO trajectories using different initialization methods with $5$KFs on the v2\_01 dataset. VIO trajectories initialized with mono-depth diverge from the ground truth far less than the baseline initialized trajectories.}
    \label{fig:vio-evaluation}
\end{figure}


==> implementation.tex <==
\subsection{Monocular Depth Estimation Model Training}
 
\subsection{Feature Matching Front End}
Our feature matching front end is quite standard like other feature based SLAM system, it includes feature extraction and feature matching between consecutive frames. Our feature extraction module is based on FREAK feature\cite{freak}. And we use 2-pt based RANSAC\cite{2-pt-ransac} for feature matching since we have IMU and we can use gyro measurements between two frames as the rotation prior.

\subsection{Visual-inertial Odometry Initialization}
The closed-form solution is solved using Eigen\cite{eigen} and the bundle adjustment refinement is formulated and solved by Levenberg Marquardt using Ceres Solver\cite{ceres-solver}.

For the bundle adjustment refinement step, we perform it in a two step way. We first perform bundle adjustment only with VI-SFM constraints. Secondly, we add inverse depth constraints and joint optimize with VI-SFM constraints. The first bundle adjustment is to maximize the benefit of outlier rejection for ML measurements. It tightens the pose solution and reduce the influence of bad poses for evaluating the standard deviation of constraint residuals in outlier rejection regardless of the scale ambiguity in which our outlier rejection can effectively deal with. We set the max iterations for the first bundle adjustment to be $18$ and set the second one to be $30$.

For inverse mono depth measurements per keyframe, we abandon those at the smallest $5\%$ inverse depth value region because those measurements could have very big uncertainty in depth.

For the $\mathcal{S}$ prior in mono depth constraints \cref{depth constraint}, we set $\sigma_a = 0.3$ and $\sigma_b = 0.2$ for scale and shift, which is very loose for covariance matrix $\Sigma_{\mathcal{S}}$. And in outlier rejection, $min_ratio$ is set to be $1.2$ while $max_ratio$ is set to be $1.45$. 

For each residual \cref{inverse depth residual}, we apply huber loss\cite{huber-loss} to improve optimization robustness. The huber factor is configured as $log(1.2)$. This means the residual is considered to be inlier when the ratio between feature point depth and recovered ML metric depth is smaller than $1.2$.


